Efficient estimates of optimal transport via low-dimensional embeddings

Optimal transport distances (OT) have been widely used in recent work in Machine Learning as ways to compare probability distributions. These are costly to compute when the data lives in high dimension. Recent work by Paty et al., 2019, aims specifically at reducing this cost by computing OT using low-rank projections of the data (seen as discrete measures). We extend this approach and show that one can approximate OT distances by using more general families of maps provided they are 1-Lipschitz. The best estimate is obtained by maximising OT over the given family. As OT calculations are done after mapping data to a lower dimensional space, our method scales well with the original data dimension. We demonstrate the idea with neural networks.

==> naturality.tex <==
\appendix
\section{Naturality} \label{naturality}
For two pseudo-metrics $\M \sim d_{\boldX}$ and $\N \sim d_{\boldY}$ on $\boldX$ and $\boldY$ respectively, we denote the probabilistic map $T$, or a deterministic one with co-domain $\boldY$. Also note that $\M \in  \setM_{\boldX}, \N \in \setM_{\boldY}$, the cone of pseudo-metrics on $\boldX,\boldY$. We will use these notations interchangeably. \\
\\
Define the pull-backward (similar to push-forward) of the pseudo-metric $\M$ on $\boldX$ through $T$ as $\tilde{T}: \N \to \M$: 
\begin{equation}\label{pullback}
\begin{aligned}
\tilde{T}(d_{\boldY})(x,x') := d_{\boldY}(T(x),T(x'))\\
\tilde{T}(\N)(x,x') := \N(T(x),T(x'))
\end{aligned}
\end{equation}



% Lipschitz
\begin{definition}\label{lipschitz}
\textbf{Lipschitz continuity} \\
$f$ is $\alpha$-Lipschitz continuous if $d_{\boldY}(f(x),f(x')) \leq \alpha d_{\boldX}(x,x')$. A 1-Lipschitz map is also called  non-expansive. For $\alpha < 1$, the map $f$ is said to be a contraction.  
\end{definition}

% Isometry
\begin{definition}\label{isometry}
\textbf{Isometry}\\
T is an isometry if $d_{\boldY}(T(x),T(x')) = d_{\boldX}(x,x')$
\end{definition}

% Lip-ISO
\begin{lemma}\label{lip-iso}
Given $u:\boldX -> \boldZ$, $u$ is $\alpha$-Lip, $u$ factors uniquely through $T$ and conversely, any factored form is Lip by composition and the fact that $T$ is an isometry. 
\end{lemma}
\begin{proof}
If $u$ is $\alpha$-Lip: 
\begin{equation}
\begin{aligned}
d_{\boldZ}(u(x), u(x')) &\leq \alpha\tilde{T}(\N)(x,x') \\
&=\alpha \N(T(x), T(x')) 
\end{aligned}
\end{equation}
\end{proof}
%
\vspace{0.5em}
We define $\tilde{T}(\N)(x,x') := \W(\N)(T(x),T(x'))$ 
and prove that criteria \eqref{eq:gml_criteria} is equivalent, in the sense of optimality for the Wasserstein distance, i.e. $\tilde{T}(\N^*)$ is best among $\tilde{T}(\N)$, by showing that  $\tup{w,G_{\tildea,\tildeb}(\N)} \leq \tup{w,G_{\bolda,\boldb}(\tilde{T}(\N))}$ with equality for $T$ deterministic. 
\begin{equation}
\W(\N)(\tildea,\tildeb) = \underset{\Delta \in U(\tildea, \tildeb)}{inf} \int_{\boldY \times \boldY}{N(y, y')d\Delta(y,y')} 
\end{equation}
\begin{equation}
\W(\tilde{T}\N)(\bolda,\boldb) = \underset{\Sigma \in U(\bolda, \boldb)}{inf} \int_{\boldX \times \boldX}{N(Tx, Tx')d\Sigma(x,x')} 
\end{equation} 
 
% Lemma 2  
\begin{lemma}\label{deterministic_metric_learning}
For $T$ deterministic, $x, x' \sim \bolda, \boldb$ and $y, y' \sim \tildea = T_{\#} \bolda  , \tildeb =  T_{\#} \boldb$ , $\W(\N)(\tildea,\tildeb) = \W(\tilde{T}\N)(\bolda,\boldb)$ holds true and $\W(\N)(\tildea,\tildeb) \leq \W(\tilde{T}\N)(\bolda,\boldb)$ for T probabilistic. \\
\\
The first statement is equivalent to the below diagram commuting, which means that the Kantorovich distance ,i.e. $\W$ is a natural transformation between the functor $\setM$ and $\setM_{P(\boldX)}$. That is a map between the functor - metrics on $\boldX$ and the functor - metrics on probabilities on $\boldX$.
\\
% Deterministic Diagram
\EQ{
\xymatrix@R=30pt@C=30pt{
\boldX\ar[d]^{T}\\
\boldY
}
&\qquad&
\xymatrix@R=30pt@C=30pt{
\setM(X) \ar[r]^{\W_{\boldX}}&
\setM_{P\boldX}
\\
\setM(Y) \ar[r]_{\W_{\boldY}}\ar[u]^{\tilde{T}}&
\setM_{P\boldY}\ar[u]_{\tilde{T}_{\#}}
}
}
\\ 
\\
The second statement is equivalent to the below diagram. \textit{F is the usual bisimulation metric} The diagram does not commute anymore, i.e. going from $\N$ to $\setM_{P\boldX}$ leaves us with a pointwise larger pseudo-metric than taking the other branch. Following the arrow can be thought of in terms of the entropic regularization previously seen. In this case we have an 'algebraic' regularization of the other branch.
% Deterministic Diagram
\EQ{
\xymatrix@R=30pt@C=30pt{
\boldX\ar[d]^{T}\\
P\boldY
}
&\qquad&
\xymatrix@R=30pt@C=30pt{
\M \ar[r]^{\W_{\boldX}}&
\setM_{P\boldX}
\\
\N \ar[r]_{\W_{\boldY}}
\ar@{.>}[u]^F&
\setM_{P\boldY}\ar[u]_{\tilde{T}^!}="A"\ar[ul]^{\tilde{T}}="B"
\ar@{:>}@/_1pc/"A";"B"
}
}


\end{lemma}
\begin{proof}
First we show that the distance over the transformation of $\boldX$ is a non-expansive map, i.e. $\W(\N)(\tildea,\tildeb) \leq \W(\tilde{T}\N)(\bolda,\boldb)$. Since T is 1-Lipschitz (or isometric?) as shown in \ref{lip-iso}, we use the dual formulation and Villani's proof \cite[\S5.4]{villani2008optimal} that shows cost functions are pseudometrics. \\ 
For $v$ Lip we have: 
%what is v? density of PX?
\begin{equation}
\begin{aligned}
\W(\tilde{T}\N)(\bolda,\boldb) &\geq \int (v \circ T) d(\bolda - \boldb) \\ 
& = \int v d(\tildea - \tildeb)
\end{aligned}
\end{equation}
which results in $\W(\tilde{T}(-)) \geq \W(-) \circ (T \times T)$. \\ 
\\ 
If $T$ has a deterministic inverse $T^*$, then couplings correspond by aggregation ($\boldY \to \boldX$) and refinement ($\boldX \to \boldY$).\\ 
In the case of finite (discrete?) optimal transport we need to compare:
If we index $x,x'$ on $\boldX$ by $i,j$ and index $k,l$ for fibers of T. 
\AR{
c_{\boldY}(i,j) &=&
\sum_{k,l} N(y_{ik},y_{jl}) \Sigma_{ik,jl}
&&
\emph{$Y$-cost of transporting $\Sigma$ on cells $i$, $j$}
\\
c_{\boldX}(i,j) &=&
\Delta_{ij}\sum_{k,l} N(y_{ik},y_{jl}) T_{ik}T_{jl}
&&\emph{aggregated $X$-cost of transport $\Delta$ on $i$, $j$}
}\\ 

If $d_{\calY}$ is the pullback of $\tilde{d_{\calY}}$, the above two are equal. More interestingly, if 
$\Sigma_{xx'} = \daggerT_{yx}\Delta_{yy'}\daggerT_{y'x'}$ results in 
$\W(\tilde{T}(-)) \geq \mbb W(-) \circ (T \times T)$

\end{proof}
\vspace{0.5em}

